Reconstructing Compact Building Models from Point Clouds Using Deep Implicit Fields

While three-dimensional (3D) building models play an increasingly pivotal role in many real-world applications, obtaining a compact representation of buildings remains an open problem. In this paper, we present a novel framework for reconstructing compact, watertight, polygonal building models from point clouds. Our framework comprises three components: (a) a cell complex is generated via adaptive space partitioning that provides a polyhedral embedding as the candidate set; (b) an implicit field is learned by a deep neural network that facilitates building occupancy estimation; (c) a Markov random field is formulated to extract the outer surface of a building via combinatorial optimization. We evaluate and compare our method with state-of-the-art methods in generic reconstruction, model-based reconstruction, geometry simplification, and primitive assembly. Experiments on both synthetic and real-world point clouds have demonstrated that, with our neural-guided strategy, high-quality building models can be obtained with significant advantages in fidelity, compactness, and computational efficiency. Our method also shows robustness to noise and insufficient measurements, and it can directly generalize from synthetic scans to real-world measurements. The source code of this work is freely available at https://github.com/chenzhaiyu/points2poly.

==> sources/4_benchmark.tex <==

\section{Dataset}

Several datasets are used to evaluate the proposed methodology. 
Due to the lack of data that contain high-quality point cloud-surface mesh pairs, we simulate our own point clouds based on the Helsinki LoD2 CityGML models\footnote{\url{https://kartta.hel.fi/3d/}}. 
Specifically, we pick 678 watertight building meshes for training, 45 for validation and another 45 for testing.
Notice that, due to the patch-based architecture for SDF learning, a large number of diverse patches 
% {\sk{how many?}} 
are produced from each mesh as training samples.

The point clouds are generated by simulated scanning on the building meshes. 
For pre-processing, the watertight building meshes are translated to the origin and scaled uniformly to unit length.
To simulate point clouds $P$ on the buildings $S$, a LiDAR sensor is configured from random perspectives. 
We use Blensor~\citep{gschwandtner2011blensor} to simulate the scanning, intentionally with various levels of Gaussian noise and artefacts such as occlusions and light reflections.

\begin{figure}[ht]
	\centering
	\subfloat[]{\includegraphics[width=0.45\linewidth]{figures/implementation/simulation_fullview.png}\label{fig:simulation_fullview}}
	\hspace{1em}
	\subfloat[]{\includegraphics[width=0.45\linewidth]{figures/implementation/simulation_nobottom.png}\label{fig:simulation_nobottom}}
	\caption[Simulation with Blensor]{Simulation with Blensor. A LiDAR scanner rotates on a sphere around the building mesh to generates a full-view point cloud (a). The scanner's position is constrained on the upper half of the sphere to simulate a no-bottom point cloud (b).}
	\label{fig:simulation}
\end{figure}

For evaluating our method against various levels of noise, we simulate multiple versions of the Helsinki dataset, each with different amounts of Gaussian noise configured. 
Various Gaussian noise simulates measurement inaccuracies onto the depth values.
We prepare point clouds with Gaussian noise whose standard deviation is randomly set in $U[0, 0.005R]$, and use this version for training the neural network.
We also create multiple versions where the Gaussian noise is fixed per dataset, from \{0, 0.001R, 0.005R, 0.010R, 0.050R\}, for evaluating the robustness of the proposed method and its competitors.

% \begin{figure}[ht]
	%   \centering
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/1_points_nonoise.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/2_points_nonoise.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/3_points_nonoise.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/4_points_nonoise.png}}
	
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/1_points_0001.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/2_points_0001.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/3_points_0001.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/4_points_0001.png}}
	
	
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/1_points_0005.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/2_points_0005.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/3_points_0005.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/4_points_0005.png}}
	
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/1_points_0010.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/2_points_0010.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/3_points_0010.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/4_points_0010.png}}
	
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/1_points_0050.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/2_points_0050.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/3_points_0050.png}}
	%   \hspace{1em}
	%   \subfloat{\includegraphics[width=0.18\linewidth]{figures/implementation/helsinki/4_points_0050.png}}
	
	%   \caption[Helsinki dataset examples]{Helsinki dataset examples. From top to bottom: Gaussian noise ranging from 0.001 to 0.050.}
	% \label{fig:helsinkiexamples}
	% \end{figure}

In addition to the simulated point clouds, the training set also contains a set of query points $X_{S}$ for each building. 
Since query points with smaller absolute distances are of higher importance for detailed surface reconstruction, we randomly sample 1000 points on the surface then apply perturbation in their normal direction by a random displacement in $U[-0.02R, 0.02R]$. 
In addition, we sample 1000 query points randomly distributed in the bounding box of the building, mounting up to 2000 query points in total per building. 
To enhance robustness of the learnt SDF, we randomly drop out 1000 query points and use the other 1000 samples for training. 
We denote this full-view dataset as \textit{Helsinki full-view}.

We further constrain the scanner's position such that no bottom view is captured and create the \textit{Helsinki no-bottom} dataset. 
The simulated point clouds resemble the real-world data of buildings acquired via multi-view stereo (MVS) or LiDAR, where rare points from the bottom of a building can be captured.
Like with \textit{Helsinki full-view}, we generate a version of point clouds with various Gaussian noise, along with the query points, as training data, and a series of point clouds with fixed noise for evaluation purpose only. 
This simulation without the bottom view is illustrated in Figure~\ref{fig:simulation_nobottom}.

Besides the synthetic data, we further evaluate our method on the real-world photogrammetric point clouds of six buildings in Shenzhen, China, produced from aerial images with MVS. 
The original images were captured by UAVs from top and lateral perspectives. 
The main bodies of buildings are visible with well-captured roof structures.
However, the building facades are only partially visible with missing areas due to occlusions and poor lighting conditions at lower part of the buildings.

\autoref{tab:datasets} summarises the characteristics of the datasets used for evaluation.
Since global shape priors are dataset-dependent, conceivably the neural network trained on one dataset may not capture the characteristics of another. 
Nonetheless, we train our neural network for SDF estimation on the \textit{Helsinki full-view} dataset and \textit{Helsinki no-bottom} dataset with various noise only, individually. 
The trained model on the former is used for evaluation on full-view point clouds, while the latter on no-bottom point clouds of typical building scans where the bottom view is not visible to the scanner.

\begin{table}[ht]
	\caption{Datasets overview}
	
	{
		\tiny
		\centering
		\begin{tabular}{lcccccc}
			\toprule
			\multirow{2}{*}{\textbf{Name}}     & \multirow{2}{*}{\textbf{Type}}   & \multicolumn{3}{c}{\textbf{Perspective}} & \multirow{2}{*}{\textbf{Quantity}} & \multirow{2}{*}{\textbf{Usage}} \\
			\cmidrule(lr){3-5}
			& & \textbf{Top} & \textbf{Bottom} & \textbf{Lateral} \\
			
			\midrule
			
			\textit{Helsinki full-view} & Simulated LiDAR       & \cmark & \cmark & \cmark            & 768               & Training + evaluation \\
			\textit{Helsinki no-bottom} & Simulated LiDAR      & \cmark  & \xmark & \cmark      & 768               & Training + evaluation \\
			\textit{Shenzhen}          & Real-world MVS & \cmark  & \xmark & \cmark     & 6                 & Evaluation            \\
			
			\bottomrule             
		\end{tabular}
	}
	
	\label{tab:datasets}
\end{table}

